Load-Altering Attacks Against Power Grids under COVID-19 Low-Inertia Conditions

The COVID-19 pandemic has impacted our society by forcing shutdowns and shifting the way people interacted worldwide. In relation to the impacts on the electric grid, it created a significant decrease in energy demands across the globe. Recent studies have shown that the low demand conditions caused by COVID-19 lockdowns combined with large renewable generation have resulted in extremely low-inertia grid conditions. In this work, we examine how an attacker could exploit these {scenarios} to cause unsafe grid operating conditions by executing load-altering attacks (LAAs) targeted at compromising hundreds of thousands of IoT-connected high-wattage loads in low-inertia power systems. Our study focuses on analyzing the impact of the COVID-19 mitigation measures on U.S. regional transmission operators (RTOs), formulating a plausible and realistic least-effort LAA targeted at transmission systems with low-inertia conditions, and evaluating the probability of these large-scale LAAs. Theoretical and simulation results are presented based on the WSCC 9-bus {and IEEE 118-bus} test systems. Results demonstrate how adversaries could provoke major frequency disturbances by targeting vulnerable load buses in low-inertia systems and offer insights into how the temporal fluctuations of renewable energy sources, considering generation scheduling, impact the grid's vulnerability to LAAs.

==> biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{subhash_lakshminarayana_profile}}]{Subhash Lakshminarayana} (S'07, M'12, SM'20) is an assistant professor at the School of Engineering, University of Warwick, UK. Previously, he worked as a researcher at the Advanced Digital Sciences Center (ADSC) in Singapore between 2015-2018, a joint post-doctoral researcher at Princeton University and the Singapore University of Technology and Design (SUTD) between 2013-2015. He received his Ph.D. from the Alcatel Lucent Chair on Flexible Radio and the Department of Telecommunications at École supérieure d'électricité, France in 2013, M.S. degree in Electrical and Computer Engineering from The Ohio State University in 2009 and B.S. from Bangalore University, India. 
His research interests include cyber-physical system security (power grids and urban transportation) and wireless communications. His works have been selected among the Best conference papers on integration of renewable \& intermittent resources at the IEEE PESGM - 2015 conference, and the ``Best 50 papers" of IEEE Globecom 2014 conference. 
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/juanj_1.jpg}}]{Juan Ospina}~(S'13-M'20) is a Postdoctoral Researcher with the A-1 Information Systems and Modeling group at Los Alamos National Laboratory (LANL). He received a dual B.Sc. degree in electrical and computer engineering and the M.S. and Ph.D. degrees in electrical engineering from Florida State University, Tallahassee, FL, USA, in 2016, 2018, and 2019, respectively. Before joining LANL, he was a Postdoctoral Researcher with the Center for Advanced Power Systems (CAPS) at Florida State University. His research interests include the development of intelligent systems for electric power systems (EPS) and smart-grid applications, machine learning and reinforcement learning models for DER control, renewable energy integration, cybersecurity of EPS, and real-time simulation.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/KonstantinouCEMSE-3.jpg}}]{Charalambos Konstantinou}~(S'11-M'18-SM'20) is an Assistant Professor of Computer Science (CS) and Affiliate Professor of Electrical and Computer Engineering (ECE) at the Computer, Electrical and Mathematical Science and Engineering Division (CEMSE) of King Abdullah University of Science and Technology (KAUST), Thuwal, Saudi Arabia. He is the Principal Investigator of the Secure Next Generation Resilient Systems Lab (SENTRY -- \href{http://sentry.kaust.edu.sa/}{sentry.kaust.edu.sa}) and a member of the Resilient Computing and Cybersecurity Center (RC3) at KAUST. His research interests are in secure, trustworthy, and resilient cyber-physical and embedded IoT systems. He is also interested in critical infrastructures security and resilience with special focus on smart grid technologies, renewable energy integration, and real-time simulation. He received a Ph.D. in Electrical Engineering from New York University (NYU), NY, in 2018, and a M.Eng. Degree in Electrical and Computer Engineering from National Technical University of Athens (NTUA), Greece, in 2012. Before joining KAUST, he was an Assistant Professor with the Center for Advanced Power Systems (CAPS) at Florida State University (FSU). Konstantinou is currently the Chair of the IEEE Task Force on Resilient and Secure Large-Scale Energy Internet Systems and the co-Chair of the IEEE Task Force on Cyber-Physical Interdependence for Power System Operation and Control. He is a Senior Member of IEEE, a member of ACM, and an ACM Distinguished Speaker (2021-2024).
\end{IEEEbiography}
